Globally Consistent Multi-People Tracking using Motion Patterns

Many state-of-the-art approaches to people tracking rely on detecting them in each frame independently, grouping detections into short but reliable trajectory segments, and then further grouping them into full trajectories. This grouping typically relies on imposing local smoothness constraints but almost never on enforcing more global constraints on the trajectories. In this paper, we propose an approach to imposing global consistency by first inferring behavioral patterns from the ground truth and then using them to guide the tracking algorithm. When used in conjunction with several state-of-the-art algorithms, this further increases their already good performance. Furthermore, we propose an unsupervised scheme that yields almost similar improvements without the need for ground truth.

==> implementation.tex <==
\section{Implementation details}
\label{sec:implementation}

Here    we   describe    the   exact    form   of    the   functions    defined
in Sec.~\ref{sec:Formulation},~\ref{sec:methodTrajectories},~\ref{sec:patterns}
followed by the details of learning and optimization. Note that our approach is
generic and can be  used with any set of functions  that follow the constraints
described in Sec.~\ref{sec:Formulation}.

\comment{\subsection{Functions}

\subsubsection{Node feature vector $f(v)$}

\pfrmk{$f$ has now disappeared from the main text. Should be reformulated or moved.}

$ f(v) = \begin{bsmallmatrix} x(v) & y(v) & t(v) & \mathds{1}(v = I) & \mathds{1}(v = O) & st(v) & fn(v) \end{bsmallmatrix}$

While features of a detection could contain more complex information such as
appearance, pose, etc., we use simple features that work even in the absence of
appearance information. We use information about the ground plane location of
the detection $l(v) = (x(v), y(v))$, the time of the detection $t(v)$, two
special features to identify special nodes $I$ and $O$, and indicators $st(v)$
and $fn(v)$ of whether detection $v$ was the beginning or ending of some
trajectory, if input was given as a set of trajectories obtained by some
approach.

\subsubsection{Edge predicate $C_e$}

We construct the set of edges to account for:

\textit{(i)} possible identity switches in the neighbouring frames:

$t(j) = t(i) + 1 \land ||l(i) - l(j)|| \le D_1 \implies (i, j) \in C_e$.

\textit{(ii)} possible trajectory fragmentations:

$t(j) \in [t(i) + 1\ldots t(i) +D_t] \land ||l(i) - l(j)|| \le D_2 \land fn(i) \land st(j) \implies (i, j) \in C_e$.

\textit{(iii)} possible false positive detection intervals:

$(I,v) \in C_e, (v, O) \in C_e \forall v \in \obj{D}$

Our construction of set of edges accounts for possible identity switches by joining the detections

No edges that don't confirm with \textit{(i)}, \textit{(ii)}, or \textit{(iii)} are constructed.
$D_1, D_2, D_t$ are the parameters controling the density of the tracking graph.

}

\paragraph  {Detection  graph  edges}   are  constructed  using  the  following
intuitive rules:  {\it i)} Each pair  of detections in the  neigibouring frames
within the distance of $D_1$ are connected by an edge to fix the possible swaps
between  identities; {\it  ii)} If  we are  given information  about the  input
trajectories,  pairs  of  last  /  first detections  in  the  trajectories  are
connected if  they are within  the distance of $D_2$  and at most  $D_t$ frames
apart  to fix  possible fragmented  trajectories; {\it  iii)} If  we are  given
information about input trajectories, transitions in them are added as edges of
detection graph to respect the results  of the input tracking method; {\it iv)}
Edges from $I$ to all detections and  from all detections to $O$ are present in
the detection graph to fix possible merged trajectories.

\paragraph  {Patterns}  $p  \in  P$  in  our  implementation  are  given  by  a
centerline  curve  $c_p:[0,1]   \to  \mathbb{R}^2$,  defined  by   one  of  the
trajectories  from the  ground truth,  and positive  width $w_p$,  as shown  by
Fig.~\ref{fig:n-and-m-functions}. When  we are  given the  ground truth  set of
trajectories and search  for patterns, each possible pattern is  defined by one
of  the  ground truth  trajectories  as  a centerline  and  some  width from  a
predefined set of possible widths.

\paragraph {For maximum possible gain function  $n(i, j, p)$} we want to ensure
that summing  it over some  trajectory $t$  gives us the  sum of the  length of
trajectory $t$ and  pattern $p$, as noted in Sec.~\ref{sec:objFunc}  (*). To do
so,  we  calculate  $n(i,  j,  p)$  as  a  sum  of  the  distance  traveled  in
trajectory  $||l(i) -  l(j)||$ and  the  appropriate distance  traveled in  the
pattern $||l_p(i)  - l_p(j)||$, where  $l(i)$ is  the ground plane  location of
detection $i$, and  $l_p(i)$ is the point on the  pattern centerline closest to
$l(i)$. Following  this logic,  $l_p(j)$ comes earlier  on the  centerline than
$l_p(i)$,  we  take the  distance  travelled  in  pattern with  negative  sign.
Fig.~\ref{fig:n-and-m-functions} provides an example.

\paragraph {For the gain function $m(i, j,  p)$} we want to ensure that summing
it  over  some trajectory  $t$  gives  us the  length  of  overlap between  $t$
and  $p$, as  noted  in Sec.~\ref{sec:objFunc}  (**). To  do  so, we  calculate
$m(i,  j,  p)$  as  a  sum  of  length  of  projection  of  $(l(i),  l(j))$  on
$(l_p(i), l_p(j))$,  denoted $(i, j)\Big{|}_{(l_p(i), l_p(j))}$,  and $(l_p(i),
l_p(j))\Big{|}_{(l(i), l(j))}$. This ensures that $m(i,  j, p) \le n(i, j, p)$,
reaching  equality if  the parts  in trajectory  and pattern  are parallel.  If
either of detections $i$ or $j$ is further from centerline $c_p$ than the width
$w_p$, $m(i, j,  p)$ is taken to  be 0 instead. If $l_p(j)$  comes earlier than
$l_p(i)$, we  take the  second term  of $m(i,  j, p)$  with negative  sign, and
multiplied by a factor of $1 + \epsilon$, to discrourage going in the direction
opposite to the pattern.

For pattern $\emptyset$ corresponding to no pattern, we take $n(i, j, p)$ to be
just the distance travelled in trajectory $||l(i)  - l(j)||$, and $m(i, j, p) =
n(i, j,  p) \epsilon_{\emptyset}$,  with $\epsilon_{\emptyset}$  controling the
likeliness of having a trajectory not following any pattern.

$n$ and  $m$ functions on the  edges from $I$ and  to $O$ take special  form to
ensure  that summing  them  over trajectory  gives the  results  we expect,  as
defined by (*) and (**). We give their exact form in supplementary materials.

\subsection{Learning}

Given a training set of trajectories $T$, we optimize the parameters
$\alpha_C, D_1, D_2, D_t, \epsilon_{\emptyset}, \epsilon$ by
cross-validation, in which we use the training part to obtain the patterns, and
the testing part to obtain the trajectories given those patterns. We then use
the optimal set of parameters to obtain the patterns on the whole training set
and trajectories on the test set.

\subsection{Implementation}

We implemented our approach in Python and C++, using Gurobi~\cite{Gurobi}
solver for solving the integer programs to find optimal set of trajectories or
patterns. We will make it publicly available upon acceptance.


